Efficient Solution of Large-Scale Algebraic Riccati Equations Associated with Index-2 DAEs via the Inexact Low-Rank Newton-ADI Method

This paper extends the algorithm of Benner, Heinkenschloss, Saak, and Weichelt: An inexact low-rank Newton-ADI method for large-scale algebraic Riccati equations, Applied Numerical Mathematics Vol.~108 (2016), pp.~125--142, doi:10.1016/j.apnum.2016.05.006 to Riccati equations associated with Hessenberg index-2 Differential Algebratic Equation (DAE) systems. Such DAE systems arise, e.g., from semi-discretized, linearized (around steady state) Navier-Stokes equations. The solution of the associated Riccati equation is important, e.g., to compute feedback laws that stabilize the Navier-Stokes equations. Challenges in the numerical solution of the Riccati equation arise from the large-scale of the underlying systems and the algebraic constraint in the DAE system. These challenges are met by a careful extension of the inexact low-rank Newton-ADI method to the case of DAE systems. A main ingredient in the extension to the DAE case is the projection onto the manifold described by the algebraic constraints. In the algorithm, the equations are never explicitly projected, but the projection is only applied as needed. Numerical experience indicates that the algorithmic choices for the control of inexactness and line-search can help avoid subproblems with matrices that are only marginally stable. The performance of the algorithm is illustrated on a large-scale Riccati equation associated with the stabilization of Navier-Stokes flow around a cylinder.

==> figures/discretized_kms_model.tex <==
\begin{tikzpicture}\footnotesize
  \node[inode,%draw=black
  ] (sym_karm) at (current page){%
    \includegraphics[width=1.01\kmslength]{./figures/kms_for_picture}};
  \node[inode,below right, xshift=.14\kmslength,yshift=-.0055\kmslength] (gin) at
  (sym_karm.north west){$\Gammain$}; 
  \node[inode,right=.101\kmslength] (gfo)
  at (gin.east){$\Gammafeed$}; 
  \node[inode,right=.058\kmslength]
  (gft) at (gfo.east){$\Gammafeed[2]$};
  \node[inode,right=.058\kmslength] (gwall) at
  (gft.east){$\Gammawall$}; 
  \node[inode,right=.09\kmslength]
  (gout) at (gwall.east){$\Gammaout$};
  \node[inode,right=.037\kmslength]
  (Pobs) at (gout.east){$\text{P}_{\text{obs},i}$};
\end{tikzpicture}

%%% Local Variables: 
%%% mode:latex
%%% mode:reftex
%%% TeX-PDF-mode:t
%%% auto-fill-function:nil
%%% mode:auto-fill
%%% flyspell-mode:nil
%%% mode:flyspell
%%% ispell-local-dictionary: "american"
%%% TeX-master: "../main.tex"
%%% End: 

